Transformer-based Ranking Approaches for Keyword Queries over Relational Databases

Relational Keyword Search (R-KwS) systems enable naive/informal users to explore and retrieve information from relational databases without requiring schema knowledge or query-language proficiency. Although numerous R-KwS methods have been proposed, most still focus on queries referring only to attribute values or primarily address performance enhancements, providing limited support for queries referencing schema elements. We previously introduced Lathe, a system that accommodates schema-based keyword queries and employs an eager CJN evaluation strategy to filter out spurious Candidate Joining Networks (CJNs). However, Lathe still faces challenges in accurately ranking CJNs when queries are ambiguous. In this work, we propose a new transformer-based ranking approach that provides a more context-aware evaluation of Query Matches (QMs) and CJNs. Our solution introduces a linearization process to convert relational structures into textual sequences suitable for transformer models. It also includes a data augmentation strategy aimed at handling diverse and ambiguous queries more effectively. Experimental results, comparing our transformer-based ranking to Lathe's original Bayesian-based method, show significant improvements in recall and R@k, demonstrating the effectiveness of our neural approach in delivering the most relevant query results.

==> algorithms/alg-CNKMIter.tex <==
\begin{algorithm}[!htb]
\caption{CJNInter($G_S,M,score_{M}$)}

\label{alg:cnkmperqmgen}

\KwIn{The query match $M$; The schema graph $G_S$
}

\KwOut{A set $C\!J\!N$ of candidate networks for the query match $M$}

$C\!J\!N \leftarrow [\ ]$\;
$J \leftarrow$ Graph() \;
\Let{$K\!M$ be an element from $M$} \label{line:cnkm-starting-node-start}

Add $K\!M$ to $J$.$\mathcal{V}$ \; \label{line:cnkm-starting-node-end}

\If{$|M|=1$}{ 
	\Return{$\{J\}$} \label{line:cnkm-unitary-cn}
}
$D \leftarrow$ queue() \; \label{line:cnkm-inicialization-start}
$D\!$.enqueue($J$) \; \label{line:cnkm-inicialization-end}
\While{$D \neq \{\}$}{ \label{line:cnkm-begin-expansion} 
	$J \leftarrow D\!$.dequeue()\;
	\For{$K\!M_u \in J.\mathcal{V}$}{
		\Let{
		    $K\!M_u$ be 
		    $R_u^{S}[A_{u,1}^{K^S_{u,1}},\ldots,A_{u,m}^{K^S_{u,m}}]^{V}[A_{u,1}^{K^V_{u,1}},\ldots,A_{u,m_u}^{K^V_{u,m_u}}]$
		}
		\Let{$G_S^U$ be the undirected version of $G_S$}
		\For{ $R_a$ adjacent to $R_u$ in $G_S^U$}{ \label{line:cnkm-undirected-schema-graph} 
			\For{$K\!M_v \in M{\setminus}C\!N\!.\mathcal{V}$}{
			    \Let{
        		    $K\!M_v$ be 
        		    $R_v^{S}[A_{v,1}^{K^S_{v,1}},\ldots,A_{v,m}^{K^S_{v,m}}]^{V}[A_{v,1}^{K^V_{v,1}},\ldots,A_{v,m_v}^{K^V_{v,m_v}}]$
        		}
			    \If{$R_v = R_a$}{
				    $J' \leftarrow J$\;				\label{line:cnkm-new-tree-start} 
    				Expand $J'$ with $K\!M_v$ joined to $K\!M_u$\; \label{line:cnkm-new-tree-end} 
    				
    				\If{$J' \notin C\!N$ \KwAnd $J'$ is \emph{sound}}{ \label{line:cnkm-check-sound} 
    					\If{$J'.\mathcal{V} \supseteq M$}{   \label{line:cnkm-check-become-cn-start} 
    						$C\!N$.append($J'$) \;  
    					}
    					\Else{
    						$D$.enqueue($J'$) \; \label{line:cnkm-check-become-cn-end}
    					}
    				}
				}
			}
			$J' \leftarrow J$\;		
			Expand $J'$ with $R_a^S[\ ]^V[\ ]$ joined to $K\!M_u$\;
			$D$.enqueue($J'$) \;
		}
	}
} \label{line:cnkm-end-expansion}
\Return{$C\!J\!N$}  \label{line:cnkm-return-results}
\end{algorithm}




==> algorithms/alg-CNKMRank.tex <==
\begin{algorithm}[htb]
	\caption{CJNKMRank($Q\!M$)}
	\label{alg:cnkmrank}
	\KwIn{A set of candidate joining networks $C\!J\!N$
	}
	\KwOut{The set of candidate networks $R\!C\!J\!N$}
	$R\!C\!J\!N \leftarrow [\ ]$\;
	\For{$C \in R\!C\!N$}{
		\Let{$M$ be the query match used to generate $C$}
		
		cjn\_score = $score(M) /|C|$
		
		$R\!C\!J\!N\!$.append( $\langle cjn\_score, C \rangle $ )
	}
	
	\textbf{Sort }$R\!C\!N$ in descending order\; \label{line:sorting}
	
	\Return{$R\!C\!J\!N$}	
\end{algorithm}


==> algorithms/alg-DelayedVKMInter.tex <==
\begin{algorithm}[!htb]

	\caption{VKMInter($P$)}
	\label{alg:VKMInter}

	\KwIn{A Hash Table $P$ whose keys are partial value-keyword matches and values are tuples.}
	\KwOut{A Hash Table $P$ whose keys are proper value-keyword matches and values are tuples.}

    \Let{$P_{next}$ be a Hash Table.} \label{VKMInter:line-begin-definition}
    \Let{$R$ be a Hash Table.}
    \For{value-keyword match $K\!M_{u} \in P $}{
	    $R[K\!M_{u}] \leftarrow \emptyset $ \;
	} \label{VKMInter:line-end-definition}
	\For{pair of keyword matches $\{K\!M_a,K\!M_b\} \in \binom{P}{2}$}{ \label{VKMInter:line-begin-intersection}
	    $K\!M_{ab} \leftarrow K\!M_{a} \cap K\!M_{b}$ \;
		$T_{ab} \leftarrow P[K\!M_a] \cap P[K\!M_b]$ \;
		\If{$T_{ab} \neq \emptyset \ \KwAnd \ K\!M_{ab}$ is valid}{ \label{VKMInter:line-if-intersection}
			$P_{next}[K\!M_{ab}] \leftarrow T_{ab}$\;
			$R[K\!M_{a}] \leftarrow R[K\!M_{a}] \cup T_{ab}$\;
			$R[K\!M_{b}] \leftarrow R[K\!M_{b}] \cup T_{ab}$\; \label{VKMInter:line-add-for-removal}
		}
	} \label{VKMInter:line-end-intersection}
	\For{value-keyword match $K\!M_{u} \in R$}{ \label{VKMInter:line-begin-removal}
	    $P[K\!M_{u}] \leftarrow P[K\!M_{u}] - R[K\!M_{u}]$ \;
	    \If{$P[K\!M_{u}] = \emptyset $}{
	        \textbf{remove } $K\!M_{u}$ from $P$\;
	        $P.remove(K\!M_{u})$ \;
	    } 
	} \label{VKMInter:line-end-removal}
	$P_{next} \leftarrow \textbf{VKMInter}(P_{next})$\; \label{VKMInter:line-next-iteration}
    \textbf{update } $P$ \textbf{with} $P_{next}$\;    \label{VKMInter:line-update-pool}
	\Return{$P$} \label{VKMInter:line-return}
\end{algorithm}



==> algorithms/alg-MergeQueryMatches.tex <==
 \begin{algorithm}[!htb]
	\caption{MergeKeywordMatches($Q,M$)}
	\label{alg:merge-keyword-matches}
	\KwIn{	The set of keyword matches $M$	}
	\KwOut{The set of keyword matches $M'$}
	\Let{$P_{V\!K}$ be a Hash Table.} \label{line:mergekms-begin-hash-generation}
	\Let{$P_{S\!K}$ be a Hash Table.}
	\For{ $K\!M \in M$}{
	    \Let{$K\!M$ be $R^{X}[A_{1}^{K_{1}},\ldots,A_{m}^{K_{m}}]$, where $X \in \{S,V\}$}
	    $P_{V\!K}[R] \leftarrow \emptyset$\;
	    $P_{S\!K}[R] \leftarrow \emptyset$\;
	}
	\For{ $K\!M \in M$}{
		\Let{$K\!M$ be $R^{X}[A_{1}^{K_{1}},\ldots,A_{m}^{K_{m}}]$,
	    where $X \in \{S,V\}$}
	     \uIf{$X = S$}{
            $P_{S\!K}[R] \leftarrow P_{S\!K}[R] \cup \{K\!M\}$\;
        }
        \Else{
            $P_{V\!K}[R] \leftarrow P_{V\!K}[R] \cup \{K\!M\}$\;
        }
	} \label{line:mergekms-end-hash-generation}
	$M' \leftarrow \emptyset$\;
	\For{$R \in P_{S\!K}$}{ \label{line:mergekms-begin-skm-merge}
	    \Let{$K\!M_{merged}$ be a keyword-free match from $R$}
	    \For{$S\!K\!M \in P_{S\!K}[R]$}{
	        $K\!M_{merged} \leftarrow K\!M_{merged} \cap S\!K\!M$\;
	    } \label{line:mergekms-end-skm-merge}
	    \If{$P_{V\!K}[R] \neq \emptyset$}{ \label{line:mergekms-begin-vkm-merge}
	        \Let{$V\!K\!M$ be an element from $P_{V\!K}[R]$}
	        $K\!M_{merged} \leftarrow K\!M_{merged} \cap V\!K\!M$\;
	        $P_{V\!K}[R] \leftarrow P_{V\!K}[R] - \{V\!K\!M\}$\;
	    } \label{line:mergekms-end-vkm-merge}
	    $M' \leftarrow M' \cup \{K\!M_{merged}\} \cup P_{V\!K}[R]$\; \label{line:mergekms-add-kmmerged}
	}
	\Return{$M'$} \label{line:mergekms-return}
\end{algorithm}

==> algorithms/alg-MinimalCover.tex <==
\begin{algorithm}[!htb]
	\caption{MinimalCover($Q,M$)}
	\label{alg:minimalCover}
	\KwIn{A keyword query $Q{=}\{k_{1},k_{2},\ldots,k_{m}\}$\newline
		The set of keyword matches $M$
	}
	\KwOut{If the set of keywords from $M$ forms a minimal cover over $Q$}
	$C_M \leftarrow \emptyset$ \; \label{line:minimalcover-begin-cover-qm}
	\For{keyword match $K\!M \in M$}{
	    \Let{$K\!M$ be $R^{X}[A_{1}^{K_{1}},\ldots,A_{m}^{K_{m}}]$,
	    where $X \in \{S,V\}$}
		\For{$i \in \{1,\ldots,m\}$}{
			$C_M \leftarrow C_M \cup K_{i}$\;
		}	
	} \label{line:minimalcover-end-cover-qm}
	\If{$ |C_M| \neq |Q|$}{ \label{line:minimalcover-check-total}
		\Return{$False$}
	}
	\For{keyword match $K\!M \in M$}{  \label{line:minimalcover-begin-cover-km}
	    \Let{$K\!M$ be $R^{X}[A_{1}^{K_{1}},\ldots,A_{m}^{K_{m}}]$,
	    where $X \in \{S,V\}$}
	    $C_{K\!M} = \emptyset$ \;
		\For{$i \in \{1,\ldots,m\}$}{
			$ C_{K\!M} \leftarrow C_{K\!M} \cup K_{i}$\;
		}	  \label{line:minimalcover-end-cover-km}
		\If{$|C_M \setminus C_{K\!M}| = Q$}{ \label{line:minimalcover-check-minimal}
			\Return{$False$}
		}
	}
	\Return{$True$}
\end{algorithm}

==> algorithms/alg-QMGen.tex <==
\begin{algorithm}[!htb]
	\caption{QMGen($Q,V\!K,S\!K$)}
	\label{alg:qmgen}
	\KwIn{A keyword query $Q{=}\{k_{1},k_{2},\ldots,k_{m}\}$ \newline
		The set of value-keyword matches $V\!K$  \newline
		The set of schema-keyword matches $S\!K$ \newline
		The maximum QM size $t$\;
		
	}
	\KwOut{The set of query matches $Q\!M$}
	$P = V\!K \cup S\!K$\;
	$Q\!M \leftarrow \emptyset$\;
	\For{$i \in \{1,\ldots,\textbf{min}(|Q|,t)\}$}{ \label{line:qmgen-iteration-max-size}
	    \For{combination of keyword matches $M \in \binom{P}{i}$}{ \label{line:qmgen-iteration-combination}
			\If{\textbf{MinimalCover}($M,Q$)}{
				$M \leftarrow $\textbf{MergeKeywordMatches($M$)} \;
				$Q\!M\! \leftarrow Q\!M\! \cup \{M\}$ \;
			}
		}
	}
	\Return{$Q\!M$}	
\end{algorithm}


==> algorithms/alg-QMRank.tex <==
\begin{algorithm}[!htb]
	\caption{QMRank($Q\!M$)}
	\label{alg:qmrank}
	\KwIn{A set of query matches $Q\!M$
	}
	\KwOut{The set of ranked query matches $R\!Q\!M$}
	$R\!Q\!M \leftarrow [\ ]$\;
	\For{$M \in Q\!M$}{
		$value\_score \leftarrow 1,$
		$schema\_score \leftarrow 1$
		
		\For{ $K\!M \in M$}{
    		\Let{
    		    $K\!M$ be 
    		    $R^{S}[A_{1}^{K^S_{1}},\ldots,A_{m}^{K^S_{m}}]^{V}[A_{1}^{K^V_{1}},\ldots,A_{m}^{K^V_{m}}]$
    		}
    	    \For{$i \in \{1,\ldots,m\}$}{
    	        \If{$|K_{i}^V| \geq 1$}{
    	            $weight\_sum \leftarrow 0$\;
    	            $norm_{A_i} \leftarrow I_S[R][A_i]$\;
    	            \For{$word \in K_{i}^V$}{
    	                $tf \leftarrow |I_V[word][R][A_i]|$\;
    	                $weight\_sum \leftarrow weight\_sum + tf\times \textbf{iaf}(word)$\;
    	            }
					$value\_score \leftarrow value\_score \times weight\_sum/norm_{A_i}$
				}
				\If{$|K_{i}^S| \geq 1$}{
    	            $weight\_sum \leftarrow 0$\;
    	            \For{$word \in K_{i}^S$}{
    	                \uIf{$A_j = self$}{
							$schema\_element \leftarrow R$
						}
						\Else{
							$schema\_element \leftarrow A_i$
						}
						$weight\_sum \leftarrow weight\_sum + \textbf{sim}(schema\_element,word)$\;
    	            }
					$schema\_score \leftarrow schema\_score \times weight\_sum/|K_{i}^S|$
				}
    	    }
    	}
		$final\_score \leftarrow value\_score \times schema\_score$\;
		$R\!Q\!M$.append($\langle final\_score, M \rangle$)
	}
	
	\textbf{Sort }$R\!Q\!M$ in descending order\; \label{line:qm-sorting}
	
	\Return{$R\!Q\!M$}	
\end{algorithm}


==> algorithms/alg-SKMGen.tex <==
\begin{algorithm}[!htb]
	\caption{SKMGen($Q$)}
	\label{alg:skmgen}
	\KwIn{A keyword query $Q{=}\{k_{1},k_{2},\ldots,k_{m}\}$, the Schema Index $I_S$}
	\KwOut{The set of schema-keyword matches $S\!K$}
	$S\!K \leftarrow \{\}$\;
	\For{keyword $k_i \in Q$}{  \label{line:skmgen-start-iteration}
		\For{relation $R_j \in I_S$}{  \label{line:skmgen-end-iteration}			
			
			\If{$sim(k_i,R_j) \geq \varepsilon$}{ \label{line:skmgen-threshold1}
			    \Let{$K\!M$ be the schema-keyword match $R_j^S[self^{\{ k_i \}}]$}
				$S\!K\! \leftarrow S\!K\! \cup \{K\!M\}$)	
			}	
			
			\For{ attribute $A_l \in I_S[R_j]$}{
				\If{$sim(k_i,A_l) \geq \varepsilon$}{ \label{line:skmgen-threshold}
				    \Let{$K\!M$ be the schema-keyword match $R_j^S[A_l^{\{ k_i \}}]$}
					$S\!K\! \leftarrow S\!K\! \cup \{K\!M\}$
				}	
			}
			
		}	
	}
	\Return{$S\!K$}
\end{algorithm}


==> algorithms/alg-SVMatCNGen.tex <==
\begin{algorithm}[htb]
	\caption{CJNGen($R\!Q\!M,G_S$)}
	\label{alg:cnkmgen}
	\KwIn{The set of ranked query matches $R\!Q\!M$  \newline
		The schema graph $G_S$
	}
	\KwOut{The set of candidate networks $C\!J\!N$}
	
	$C\!J\!N = \{\}$\;
	\For{query match $M \in R\!Q\!M$}{
		$C\!J\!N_M \leftarrow$ \textbf{CJNInter}($M,G_S$)\;	
		$C\!J\!N \leftarrow C\!J\!N \cup C\!J\!N_M$
	}
	\Return{$C\!J\!N$}
\end{algorithm}


==> algorithms/alg-SVSingleCNGen.tex <==
\begin{algorithm}[!htb]
\caption{CNKMInter($M,G_S$)}

\label{alg:cnkmperqmgen}

\KwIn{The query match $M$; The schema graph $G_S$
}

\KwOut{A set $C\!N$ of candidate networks for the query match $M$}

\Let{$G_S^U$ be the undirected version of $G_S$}

\Let{$K\!M$ be an element from $M$} \label{line:cnkm-starting-node-start}
$C\!N \leftarrow [\ ]$ \;

$C \leftarrow$ graph() \;

Add $K\!M$ to $C$.$\mathcal{V}$ \; \label{line:cnkm-starting-node-end}

\If{$|M|=1$}{ 
	\Return{$\{C\}$} \label{line:cnkm-unitary-cn}
}
$D \leftarrow$ queue() \; \label{line:cnkm-inicialization-start}
$D\!$.enqueue($C$) \; \label{line:cnkm-inicialization-end}
\While{$D \neq \{\}$}{ \label{line:cnkm-begin-expansion} 
	$C \leftarrow D\!$.dequeue()\;
	
	\ForEach{keyword match $K\!M_u \in C\!N\!.\mathcal{V}$}{
		\Let{$R_u$ be the relation of $K\!M_u$}
		\For{ relation $R_a$ adjacent $R_u$ in $G_S^U$}{ \label{line:cnkm-undirected-schema-graph} 
			\For{keyword match $K\!M_v \in M \setminus C\!N\!.\mathcal{V} | R_v = R_a$}{
				$C' \leftarrow C$\;				\label{line:cnkm-new-tree-start} 
				Expand $C'$ with $K\!M_v$ joined to $K\!M_u$\; \label{line:cnkm-new-tree-end} 
				
				\If{$C' \notin C\!N$ \KwAnd $C'$ is \emph{sound}}{ \label{line:cnkm-check-sound} 
					\If{$C'.\mathcal{V} \supseteq M$}{   \label{line:cnkm-check-become-cn-start} 
						$C\!N$.append($C'$) \;  
					}
					\Else{
						$D$.enqueue($C'$) \; \label{line:cnkm-check-become-cn-end}
					}
				}
			}
			$C' \leftarrow C$\;				
			Expand $C'$ with the keyword-free match $R_a^S[\ ]^V[\ ]$ joined to $K\!M_u$\;
			$D$.enqueue($C'$) \;
		}
	}
} \label{line:cnkm-end-expansion}
\Return{$C\!N$}  \label{line:cnkm-return-results}
\end{algorithm}




==> algorithms/alg-SoundCN.tex <==
\begin{algorithm}[!htb]
	\caption{isJPSound($G_S$,$J'$)}
	\label{alg:isjpsound}
	\KwIn{The schema graph $G_S$ \newline 
		The join path $J'$ in $G_S$}
	\KwOut{Whether the join path $J'$ is sound.}
	
	\If{$|J'|<3$}{
		\Return{$True$}
	}
	
	\For{$i \in \{1,\ldots, |J'|-2\}$}{
		\If{$relation(J'[i]) = relation(J'[i+2])$}{
			\If{RIC($relation(J'[i],J'[i+1])$}{
				\tcc{Unsound case: $R_a \longleftarrow R_{b} \longrightarrow R_{a}$}
				\Return {$False$}
			}
		}
	}
	\Return{$True$}	
\end{algorithm}




==> algorithms/alg-VKMGen.tex <==
\begin{algorithm}[!htb]
	\caption{VKMGen($Q$)}
	\label{alg:vkmgen}
	\KwIn{A keyword query $Q{=}\{k_{1},k_{2},\ldots,k_{m}\}$}
	\KwOut{The set of value-keyword matches $V\!K$}
	
	\Let{$I_V$ the Value Index}
    \Let{$P\!$ be a Hash Table.}
	\For{keyword $k_i \in Q$}{ \label{line:vkmgen-begin-for}
		\If{$k_i \in I_V$}{
			\For{relation $R_j \in I_V[k_i]$}{
				\For{ attribute $A_k \in I_V[k_i][R_j]$}{
				    \Let{$K\!M$ be the partial keyword match $R_j^V[A_k^{\{ k_i \}}]$}
					$P[K\!M] \leftarrow I_V[k_i][R_j][A_k]$ \label{line:vkmgen-conversion}
				}
			}	
		}
	}
	$P \leftarrow \textbf{VKMIter}(P$) \; \label{VKMGen-line-recursive-call}
	\For{value-keyword match $K\!M_{u} \in P$}{ \label{VKMGen-line-begin-ignore-tuple}
	    $V\!K \leftarrow V\!K \cup \{K\!M_{u}\}$ \;
	} \label{VKMGen-line-end-ignore-tuple}
	\Return $V\!K$	
\end{algorithm}


==> algorithms/alg-VKMInter.tex <==
\begin{algorithm}[!htb]

	\caption{VKMInter($VK$)}
	\label{alg:VKMInter}

	\KwIn{A set of value-keyword matches $V\!K$}

	\For{pair of value-keyword matches $\{K\!M_a,K\!M_b\} \in \binom{V\!K}{2}$}{

		$K\!M_{ab} \leftarrow K\!M_a \cap K\!M_b$

		

		\If{$K\!M_{ab} \neq \{\} \ \KwAnd \ K\!M_{ab}$ is valid}{

			

			$V\!K\!$.append($K\!M_{ab}$)

			

			$K\!M_{a} \leftarrow K\!M_{a} - K\!M_{ab}$

			

			\uIf{$K\!M_{a} = \{\}$}{

				$V\!K\!$.remove($K\!M_{a}$)	

			}

			\Else{

				$V\!K\!$.update($K\!M_{a}$)

			}			

			$K\!M_{b} \leftarrow K\!M_{b} - K\!M_{ab}$

			

			\uIf{$K\!M_{b} = \{\}$}{

				$V\!K\!$.remove($K\!M_{b}$)	

			}

			\Else{

				$V\!K\!$.update($K\!M_{b}$)

			}

			

			\textbf{VKMInter($V\!K$)}

		}
	}
\end{algorithm}



==> snippets/exverbis_SQL_enhanced.tex <==
\begin{lstlisting}
SELECT COUNT(DISTINCT p.title)
FROM publications p
JOIN writes w ON w.pid=p.pid
JOIN authors a ON a.aid=w.aid
JOIN conferences c ON c.cid=p.cid
WHERE a.name ILIKE '%h.v.jagadish%'
AND c.name ILIKE '%vldb%' 
AND p.year>2000
AND p.citation_num>200
\end{lstlisting} 

==> snippets/exverbis_SQL_vanilla.tex <==
\begin{lstlisting}
SELECT p.title, a.name, c.name, 
p.year, p.citation_num
FROM publications p
JOIN writes w ON w.pid=p.pid
JOIN authors a ON a.aid=w.aid
JOIN conferences c ON c.cid=p.cid
WHERE a.name ILIKE '%h.v.jagadish%'
AND c.name ILIKE '%vldb%' 
AND p.year = 2000
\end{lstlisting} 

==> snippets/sereia_mongo_query.tex <==
\begin{lstlisting}[language=json]
db.user.aggregate([
{ "$match": { "$expr": { "$regexMatch": { 
    "input": "$user.name", "regex": "michelle", 
    "options": "i"}}}},
{ "$lookup": { "from": "review", "foreignField": "user_id", 
               "localField": "user_id", "as": "review"}},
{ "$unwind": "$review" },
{ "$lookup": { "from": "business", "foreignField": "business_id", 
               "localField": "review.business_id", "as": "business"}},
{ "$unwind": "$business" },
{ "$match": { "$expr": { "$regexMatch": { 
    "input": "$categories", "regex": "restaurants", 
    "options": "i"}}},
{ "$match": { "$expr": { "$regexMatch": { 
    "input": "$categories", "regex": "italian", 
    "options": "i"}}}}])
\end{lstlisting}

==> tables/demo_tab_cast.tex <==
\begin{tabular}{|c|c|c|}
	\multicolumn{3}{@{}l}{\textbf{CASTING} } 
	\\ 
	\hline
	
	\textbf{ID}
	& \textbf{PID} 
	& \textbf{MID}
	\\ 
	
	\hline
	
	\deftupleno{jr-mc}
	&\reftupleno{jr}
	&\reftupleno{mc}\\
	
	\deftupleno{rj-rookie}
	&\reftupleno{rj}
	&\reftupleno{rookie}\\
	
	\deftupleno{rh-rookie}
	&\reftupleno{rh}
	&\reftupleno{rookie}\\
	
	\multicolumn{1}{|c|}{\rvdots}
	& \multicolumn{1}{c|}{\rvdots}
	& \multicolumn{1}{c|}{\rvdots}
	\\
	
	\hline
\end{tabular}

==> tables/demo_tab_movie.tex <==
% Size for two column
% \begin{tabularx}{1.08\columnwidth}{r@{}|c|X|l|}
\begin{tabular}{|c|l|c|}
    \multicolumn{3}{@{}l}{\textbf{MOVIE}}\\ 
	\hline

	\textbf{ID}
	& \textbf{Title}
	& \textbf{Year}\\ 
	\hline
	
	\deftupleno{mc}
	& Michael Collins
	& 1996\\
	
	\deftupleno{rookie}
	& The Rookie
	& 1990\\
	
	\deftupleno{pw}
	& Pretty Woman
	& 1996\\
	
	\multicolumn{1}{|c|}{\rvdots}
	& \multicolumn{1}{c|}{\rvdots}
	& \multicolumn{1}{c|}{\rvdots}
	\\
    \hline
% 	\multicolumn{1}{l}{}
% 	& \multicolumn{1}{l}{}
\end{tabular}

==> tables/demo_tab_person.tex <==
\begin{tabular}{|c|l|}
	\multicolumn{2}{@{}l}{\textbf{PERSON}}\\
	\hline
	
	\textbf{ID}
	& \textbf{Name}\\
	\hline
	
	\deftupleno{jr}
	& Julia Roberts\\
	
	\deftupleno{rj}
	& Raul Julia\\
	
	\deftupleno{rh}
	& Robert Harvey\\
	
    \multicolumn{1}{|c|}{\rvdots}
	& \multicolumn{1}{c|}{\rvdots}
	\\
	\hline
\end{tabular}

==> tables/schema_labeling_tab1.tex <==
\begin{tabular}{|l|l|l|l|c|l|c|}
\hline
\textbf{A1}       & \textbf{A2} & \textbf{A3} & \textbf{A4} & \textbf{A5} & \textbf{A6} & \textbf{A7} \\ \hline
Cristiano Ronaldo & 02/05/1985  & Portugal    & Juventus    & 29          & forward     & 7           \\ \hline
Lionel Messi      & 06/24/1987  & Argentina   & Barcelona   & 34          & forward     & 10          \\ \hline
Sergio Ramos      & 03/30/1986  & Spain       & Real Madrid & 21          & defense     & 4           \\ \hline
\end{tabular}

==> tables/tab-datasets.tex <==
\begin{tabular}{lrrrrr} 
	\toprule
	Dataset & Size(MB) & Relations &  Attributes & RIC & Tuples     \\ 
	\midrule
	MONDIAL & 13        & 28  & 48       & 38  & 17,115     \\
	IMDb    & 528      &    6  & 33     & 5   & 1,673,076 
\\
	\bottomrule
\end{tabular}

==> tables/tab-querysets.tex <==
\begin{tabular}{cc}
	\small
	\begin{tabular}{llccc}
		\toprule
		\normalsize Dataset &
		\normalsize Queryset &
		\normalsize $|Q|$ &
		\normalsize $|s|$ &
		\normalsize $|a|$ \\
		\midrule
		
		\normalsize IMDb &
		\normalsize Coffman &
		\normalsize 50 &
		\normalsize 20&
		\normalsize 5  \\
		
		\normalsize IMDb &
		\normalsize Coffman-CI &
		\normalsize 50 &
		\normalsize 25&
		\normalsize -  \\
		
		\normalsize MONDIAL &
		\normalsize Coffman &
		\normalsize 45 &
		\normalsize 12&
		\normalsize 7  \\
		
		\normalsize MONDIAL &
		\normalsize Coffman-CI&
		\normalsize 45 &
		\normalsize 19&
		\normalsize -  \\
		
		\midrule
	\end{tabular} 
	&
	\begin{tabular}{cl}
		\multicolumn{2}{l}{\textbf{Legend}} \\
		$|Q|$ &
		total number of queries \\
		
		$|s|$ &
		total number of schema references \\
		
		$|a|$ &
		total number of ambiguous queries \\
		
		x-CI &
		queryset x with queries desambiguated\\
		& with schema references
	\end{tabular}
\end{tabular}


==> tables/tab_CN1_SQL_RESULT.tex <==
\begin{tabular}{cc}
	\begin{lstlisting}
	SELECT p.id,p.name,c.id,m.id,m.title
	FROM person p 
	JOIN casting c ON p.id=c.person_id
	JOIN movie m ON c.movie_id=m.id
	WHERE p.name ILIKE '%will%'
	AND p.name ILIKE '%smith%';
	\end{lstlisting} 
	&
	\begin{tabular}{|c|l|c|c|l|} 
	\hline
	\textbf{p.id} & \textbf{p.name} &\textbf{c.id} & \textbf{m.id} &\textbf{m.title}\\ 
	\hline
	$\reftupleno{ws}$ & Will Smith & $\reftupleno{ws-mib-agentj}$ & $\reftupleno{mib}$ & Men in Black\\
	\hline
	$\reftupleno{ws}$ & Will Smith & $\reftupleno{ws-legend-neville}$ & $\reftupleno{legend}$ & I am Legend\\
	\hline
	\end{tabular}
	\\
	(a) & (b) 
\end{tabular}

==> tables/tab_CN2_1_SQL_RESULT.tex <==
\begin{tabular}{cc}
	\begin{lstlisting}
	SELECT p1.id,p1.name,c1.id,m.id,m.title,
		c2.id,p2.id,p2.name
	FROM person p1 
	JOIN casting c1 ON p1.id=c1.person_id
	JOIN movie m ON c1.movie_id=m.id
	JOIN casting c2 ON m.id=c2.movie_id
	JOIN person p2 ON c2.person_id=p2.id
	WHERE p1.name ILIKE '%will%'
		AND p2.name ILIKE '%smith%'
		AND __p1.id<>p2.id__
		AND __c1.id<>c2.id__;
	\end{lstlisting}
	&
	\begin{tabular}{|c|p{2cm}|c|c|p{4cm}|c|c|p{1.5cm}|} 
		\hline
		\textbf{p1.id} & \textbf{p1.name} & \textbf{c1.id} & \textbf{m.id} & \textbf{m.title} & \textbf{c2.id} & \textbf{p2.id} & \textbf{p2.name} \\ 
		\hline
		$\reftupleno{wt}$  &Will Theakston  & $\reftupleno{wt-hp1-flint}$  & $\reftupleno{hp1}$  & Harry Potter and the Sorcerer's Stone  & $\reftupleno{ms-hp1-minerva}$ & $\reftupleno{ms}$  & Maggie Smith\\
		\hline
	\end{tabular}
	\\
	(a) & (b)
\end{tabular}

==> tables/tab_J3_SQL_queries.tex <==
\begin{tabular}{cc}
	\begin{lstlisting}
	SELECT m.title,c1.id,p.name,c2.id,ch.name
	FROM movie m
	JOIN casting c1 ON m.id = c1.movie_id
	JOIN person p ON p.id=c1.person_id
	JOIN casting c2 ON p.id = c2.person_id
	JOIN character ch ON ch.id=c2.char_id
	WHERE m.title ILIKE '%lord%'
	AND m.title ILIKE '%rings%'
	AND c1.id<>c2.id;
	\end{lstlisting} 
	&
	\begin{tabular}{|c|p{5cm}|c|c|l|c|c|l|} 
		\hline
		\textbf{m.id} & \textbf{m.title} & \textbf{c1.id} &\textbf{p.id} & \textbf{p.name} & \textbf{c2.id} &  \textbf{ch.id} &\textbf{ch.name} \\ 
		\hline
		
		\reftupleno{lotr1} & The Lord of the Rings: The Fellowship of the Ring  & \reftupleno{sb-lotr1-boromir}  & \reftupleno{sb} & Sean Bean  & \reftupleno{sb-sh-chris}&  \reftupleno{chris} & Christopher da Silva\\
		\hline
		
		\reftupleno{lotr1} & The Lord of the Rings: The Fellowship of the Ring  & \reftupleno{sb-lotr1-boromir}  & \reftupleno{sb} & Sean Bean  & \reftupleno{sb-lotr2-boromir}&  \reftupleno{boromir} & Boromir\\
		\hline
		
		\reftupleno{lotr2} & The Lord of the Rings: The Return of the King  & \reftupleno{sb-lotr2-boromir}  & \reftupleno{sb} & Sean Bean  &
		\reftupleno{sb-lotr1-boromir}  &  \reftupleno{boromir} & Boromir\\
		\hline
		\reftupleno{lotr1} & The Lord of the Rings: The Fellowship of the Ring  & \reftupleno{ew-lotr1-frodo}  & \reftupleno{ew} & Elijah Wood  &
		\reftupleno{ew-lotr2-frodo}  & \reftupleno{frodo} & Frodo Baggins\\
		\hline
		\reftupleno{lotr2} & The Lord of the Rings: The Return of the King  & \reftupleno{ew-lotr2-frodo}  & \reftupleno{ew} & Elijah Wood  & \reftupleno{ew-lotr1-frodo}  &\reftupleno{frodo} & Frodo Baggins\\
		\hline
	\end{tabular}	
	\\
	(a) & (b) \\\\
	\begin{lstlisting}
	SELECT m.title,c.id,p.name,ch.name
	FROM movie m
	JOIN casting c ON m.id = c.movie_id
	JOIN person p ON p.id=c.person_id
	JOIN character ch ON ch.id=c.char_id
	WHERE m.title ILIKE '%lord%'
	AND m.title ILIKE '%rings%';
	\end{lstlisting}
	&
	\begin{tabular}{|c|p{5cm}|c|c|l|c|l|} 
		\hline
		\textbf{m.id} & \textbf{m.title} & \textbf{c1.id} &\textbf{p.id} & \textbf{p.name} &  \textbf{ch.id} &\textbf{ch.name} \\ 
		\hline
		\reftupleno{lotr1} & The Lord of the Rings: The Fellowship of the Ring  & \reftupleno{sb-lotr1-boromir}  & \reftupleno{sb} & Sean Bean  & \reftupleno{boromir} & Boromir\\
		\hline
		\reftupleno{lotr2} & The Lord of the Rings: The Return of the King  & \reftupleno{sb-lotr2-boromir}  & \reftupleno{sb} & Sean Bean  & \reftupleno{boromir} & Boromir\\
		\hline
		\reftupleno{lotr1} & The Lord of the Rings: The Fellowship of the Ring  & $\reftupleno{sb-lotr1-boromir}$  & \reftupleno{ew} & Elijah Wood  & \reftupleno{frodo} & Frodo Baggins\\
		\hline
		\reftupleno{lotr2} & The Lord of the Rings: The Return of the King  & $\reftupleno{sb-lotr2-boromir}$  & \reftupleno{ew} & Elijah Wood  & \reftupleno{frodo} & Frodo Baggins\\
		\hline
	\end{tabular}
	\\
	(c) & (d) \\
\end{tabular}

==> tables/tab_J3_SQL_redundant.tex <==
\begin{tabular}{cc}
	\begin{lstlisting}
	SELECT m.id,m.title,c1.id,p.id,p.name,
		c2.id,ch.id,ch.name
	FROM movie m
	JOIN casting c1 ON m.id = c1.movie_id
	JOIN person p ON p.id=c1.person_id
	JOIN casting c2 ON p.id = c2.person_id
	JOIN character ch ON ch.id=c2.char_id
	WHERE m.title ILIKE '%legend%';
	\end{lstlisting}
	&
	\begin{tabular}{|c|l|c|c|l|c|c|l|} 
		\hline
		\textbf{m} & \textbf{m.title} & \textbf{c1} &\textbf{p} & \textbf{p.name} & \textbf{c2} & \textbf{ch} &\textbf{ch.name} \\ 
		\hline
		$t_7$ & I am Legend   & $t_{24}$  & $t_1$ &  Will Smith  & $t_{23}$ & $t_{11}$ & Agent J\\
		\hline
		$t_7$ &I am Legend   & $t_{24}$
		   & $t_1$ & Will Smith  & $t_{24}$ & $t_{12}$ & Robert Neville\\
		\hline
	\end{tabular}
	\\
	(a) & (b) \\
\end{tabular}

==> tables/tab_SQL_1.tex <==
\begin{tabular}{|l|l|} 
	\hline
	\textbf{m.title} & \textbf{p.name}  \\ 
	\hline
	Men in Black     & Will Smith       \\
	\hline
	I am Legend      & Will Smith       \\
	\hline
\end{tabular}

==> tables/tab_SQL_2.tex <==
\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.2cm}|} 
	\hline
	\textbf{m.title}
	& \textbf{p1.name}
	& \textbf{p2.name}  
	\\ 
	\hline
	Harry Potter and the Sorcerer's Stone 
	& Will Theaskton
	& Maggie Smith
	\\
	\hline
\end{tabular}

==> tables/tab_SQL_listing1.tex <==
\begin{lstlisting}
SELECT m.title, p.name
FROM person p
JOIN casting c ON  p.id=c.pid
JOIN movie m ON m.id = c.mid
WHERE p.name ILIKE '%will%' 
AND p.name ILIKE '%smith%';
\end{lstlisting} 

==> tables/tab_SQL_listing2.tex <==
\begin{lstlisting}
	SELECT m.title, p1.name, p2.name
	FROM person p1
	JOIN casting c1 ON p1.id=c1.pid
	JOIN movie m ON m.id = c1.mid
	JOIN casting c2 ON m.id = c2.mid
	JOIN person p2 ON p2.id=c2.pid
	WHERE p1.name ILIKE '%will%' 
	AND p2.name ILIKE '%smith%'
	AND p1.id<>p2.id;
\end{lstlisting}

==> tables/tab_border.tex <==
\begin{tabular}{rccc}
& \multicolumn{3}{l}{\textbf{BORDER}}                                                                                                \\ 
% \cline{2-4} 
\hhline{~---}
\multicolumn{1}{r|}{}                                   & \multicolumn{1}{c|}{\textbf{Ctry1\_Code}} & \multicolumn{1}{c|}{\textbf{Ctry2\_Code}} & \multicolumn{1}{c|}{\textbf{Length}} \\ 
% \cline{2-4} 
\hhline{~---}
\multicolumn{1}{r|}{\deftuple{co_br}} & \multicolumn{1}{c|}{CO}                      & \multicolumn{1}{c|}{BR}                      & \multicolumn{1}{c|}{1643}            \\
\multicolumn{1}{r|}{\deftuple{pe_br}} & \multicolumn{1}{c|}{PE}                      & \multicolumn{1}{c|}{BR}                      & \multicolumn{1}{c|}{1560}            \\
% \cline{2-4} 
\hhline{~---}
\\
\end{tabular}

==> tables/tab_casting_person_casting.tex <==
\begin{tabular}{|c|c|l|c|}
	\hline
	\textbf{c1} & \textbf{p} & \textbf{p.name} & \textbf{c2} \\ \hline
	$t_{23}$    & $t_{1}$    & Will Smith      & $t_{23}$    \\ \hline
	$t_{23}$    & $t_{1}$    & Will Smith      & $t_{24}$    \\ \hline
	$t_{24}$    & $t_{1}$    & Will Smith      & $t_{23}$    \\ \hline
	$t_{24}$    & $t_{1}$    & Will Smith      & $t_{24}$    \\ \hline
	$t_{25}$    & $t_{2}$    & Will Theakston  & $t_{25}$    \\ \hline
	$t_{26}$    & $t_{3}$    & Maggie Smith    & $t_{26}$    \\ \hline
	$t_{27}$    & $t_{4}$    & Sean Bean       & $t_{27}$    \\ \hline
	$t_{27}$    & $t_{4}$    & Sean Bean       & $t_{28}$    \\ \hline
	$t_{28}$    & $t_{4}$    & Sean Bean       & $t_{27}$    \\ \hline
	$t_{28}$    & $t_{4}$    & Sean Bean       & $t_{28}$    \\ \hline
	$t_{29}$    & $t_{5}$    & Elijah Wood     & $t_{29}$    \\ \hline
	$t_{29}$    & $t_{5}$    & Elijah Wood     & $t_{30}$    \\ \hline
	$t_{30}$    & $t_{5}$    & Elijah Wood     & $t_{29}$    \\ \hline
	$t_{30}$    & $t_{5}$    & Elijah Wood     & $t_{30}$    \\ \hline
\end{tabular}

==> tables/tab_city.tex <==
\begin{tabular}{rccc}
                      & \multicolumn{3}{l}{\textbf{CITY}}                                                                                \\ 
% \cline{2-4} 
\hhline{~---}
\multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Population}} \\ 
% \cline{2-4} 
\hhline{~---}
\multicolumn{1}{r|}{\deftuple{bogota}} & \multicolumn{1}{c|}{1}          & \multicolumn{1}{c|}{Bogota}        & \multicolumn{1}{c|}{1643}                \\
\multicolumn{1}{r|}{\deftuple{brasilia}} & \multicolumn{1}{c|}{2}          & \multicolumn{1}{c|}{Brasilia}      & \multicolumn{1}{c|}{1560}                \\
\multicolumn{1}{l|}{\deftuple{lima}} & \multicolumn{1}{c|}{3}          & \multicolumn{1}{c|}{Lima}          & \multicolumn{1}{c|}{1560}                \\ 
% \cline{2-4} 
\hhline{~---}
\end{tabular}

==> tables/tab_country.tex <==
\begin{tabular}{rcll}
    & 
    \multicolumn{3}{l}{
        \textbf{COUNTRY}
    }                                                                            
    \\
    % \cline{2-4} 
    \hhline{~---}
    \multicolumn{1}{r|}{}
    &
    \multicolumn{1}{c|}{
        \textbf{Code}
    } 
    &
    \multicolumn{1}{l|}{
        \textbf{Name}
    }
    &
    \multicolumn{1}{c|}{
        \textbf{Capital\_ID}
    }
    \\
    % \cline{2-4} 
    \hhline{~---}
\multicolumn{1}{r|}{\deftuple{colombia}} & \multicolumn{1}{c|}{CO}            & \multicolumn{1}{l|}{Colombia}      & \multicolumn{1}{c|}{1}           \\
\multicolumn{1}{r|}{\deftuple{brazil}}   & \multicolumn{1}{c|}{BR}            & \multicolumn{1}{l|}{Brazil}        & \multicolumn{1}{c|}{2}         \\
\multicolumn{1}{r|}{\deftuple{peru}}     & \multicolumn{1}{c|}{PE}            & \multicolumn{1}{l|}{Peru}          & \multicolumn{1}{c|}{3}             \\ 
% \cline{2-4} 
\hhline{~---}
\end{tabular}

==> tables/tab_deepcontext_examples.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|}
\cline{1-3} \cline{5-7}
\textbf{title}                       & \textbf{manf./modelno} & \textbf{price} & \textbf{} & \textbf{title}                & \textbf{manf./modelno} & \textbf{price} \\ \cline{1-3} \cline{5-7} 
instant immersion spanish deluxe 2.0 & topics entertainment   & 49.99          &   \tikz{\draw[OliveGreen,{Latex[length=2.2mm,width=2.2mm]}-{Latex[length=2.2mm,width=2.2mm]}] (-2,0) -- node[above] {\cmark} ++(1,0);} & instant immers spanish dlux 2 & NULL                   & 36.11          \\ \cline{1-3} \cline{5-7} 
\begin{tabular}[c]{@{}c@{}}adventure workshop 4th-6th\\ grade 7th edition\end{tabular} &
  encore software &
  19.99 &
    \tikz{\draw[red,{Latex[length=2.2mm,width=2.2mm]}-{Latex[length=2.2mm,width=2.2mm]}] (-2,0) -- node[above] {\xmark} ++(1,0);} 
   &
  \begin{tabular}[c]{@{}c@{}}encore inc adventure workshop\\ 4th-6th grade 8th edition\end{tabular} &
  NULL &
  17.1 \\ \cline{1-3} \cline{5-7} 
sharp printing calculator &
  sharp el1192bl &
  37.63 &
   \tikz{\draw[OliveGreen,{Latex[length=2.2mm,width=2.2mm]}-{Latex[length=2.2mm,width=2.2mm]}] (-2,0) -- node[above] {\cmark} ++(1,0);}
   &
  \begin{tabular}[c]{@{}c@{}}new-sharp shr-el1192bl two-color\\ printing calculator 12-digit lcd black red\end{tabular} &
  NULL &
  56.0 \\ \cline{1-3} \cline{5-7} 
\end{tabular}

==> tables/tab_general_results.tex <==
% \begin{tabular}{l|r|r|r|r|r|r|r|r|}
% \cline{2-9}
% \textbf{}                        & \multicolumn{2}{c|}{\textbf{Num. KMs}}              & \multicolumn{2}{c|}{\textbf{Num. QMs}}              & \multicolumn{2}{c|}{\textbf{Num. CNs}}              & \multicolumn{2}{l|}{\textbf{Num. JNKMs}}            \\ \hline
% \multicolumn{1}{|l|}{Query sets} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg} \\ \hline
% \multicolumn{1}{|l|}{IMDb}       & 47                       & 15.38                    & 515                      & 72.46                    & 554                      & 89.04                    & 36222                    & 5370.02                  \\ \hline
% \multicolumn{1}{|l|}{IMDb-DI}    & 64                       & 16.20                    & 515                      & 69.76                    & 492                      & 85.28                    & 34185                    & 5102.66                  \\ \hline
% \multicolumn{1}{|l|}{MOND}       & 8                        & 3.16                     & 9                        & 2.11                     & 33                       & 6.96                     & 9106                     & 2540.51                  \\ \hline
% \multicolumn{1}{|l|}{MOND-DI}    & 8                        & 3.47                     & 9                        & 2.47                     & 34                       & 7.87                     & 9529                     & 2572.13                  \\ \hline
% \end{tabular}

\begin{tabular}{|l|r|r|r|r|r|r|}
%\cline{2-9}
\hline
~ & \multicolumn{2}{c|}{\textbf{Num. KMs}} & \multicolumn{2}{c|}{\textbf{Num. QMs}}  & \multicolumn{2}{c|}{\textbf{Num. CJNs}}   \\ \hline
\multicolumn{1}{|l|}{Query sets} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c|}{Avg}  \\ \hline
\multicolumn{1}{|l|}{IMDb}    & 47   & 15.38 & 515 & 72.46 & 554 & 89.04 \\ \hline
\multicolumn{1}{|l|}{IMDb-DI} & 64   & 16.20 & 515 & 69.76 & 492 & 85.28 \\ \hline
\multicolumn{1}{|l|}{MOND}    & 8    & 3.16  & 9   &  2.11 & 33  & 6.96  \\ \hline
\multicolumn{1}{|l|}{MOND-DI} & 8    & 3.47  & 9   &  2.47 & 34  & 7.87  \\ \hline
\end{tabular}

==> tables/tab_person_casting_person.tex <==
\begin{tabular}{|c|l|c|c|l|}
	\hline
	\textbf{p1}  & \textbf{p1.name}  & \textbf{c1}  & \textbf{p2}  & \textbf{p2.name}  \\ 
	\hline
	$t_{1}$       & Will Smith        & $t_{23}$     & $t_{1}$      & Will Smith        \\ 
	\hline
	$t_{1}$       & Will Smith        & $t_{24}$     & $t_{1}$      & Will Smith        \\ 
	\hline
	$t_{2}$       & Will Theakston    & $t_{25}$     & $t_{2}$      & Will Theakston    \\ 
	\hline
	$t_{3}$       & Maggie Smith      & $t_{26}$     & $t_{3}$      & Maggie Smith      \\ 
	\hline
	$t_{4}$       & Sean Bean         & $t_{27}$     & $t_{4}$      & Sean Bean         \\ 
	\hline
	$t_{4}$       & Sean Bean         & $t_{28}$     & $t_{4}$      & Sean Bean         \\ 
	\hline
	$t_{5}$       & Elijah Wood       & $t_{29}$     & $t_{5}$      & Elijah Wood       \\ 
	\hline
	$t_{5}$       & Elijah Wood       & $t_{30}$     & $t_{5}$      & Elijah Wood       \\
	\hline
\end{tabular}

==> tables/tab_singleqjp_m1.tex <==
{\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|c|l|l|} 
		\hline
		\textbf{ I\# } &
		\textbf{Queue } &
		\textbf{Operations } \\ 
		\hline
		
		$T_1$ &
		\tikz{
			\node[main node] (1) {$PERSON^V[name^{ \{will,smith\} }]$};
		} 
		& 
		initialize, enqueue $0$ \\
		 
		\hline 
		$T_2$ & 
		\tikz{
			\node[main node] (1) {$PERSON^V[name^{ \{will,smith\} }]$};
			\node[main node] (2) [right = 3mm of 1] {$CASTING$};
			\path[draw,thick,->]
			(2) edge node {} (1)
		} 
		 & 
		 expand $0$, enqueue $1$ \\
		
		\hline
		 
		$T_3$&
		\tikz{
			\node[main node] (1) {$PERSON^V[name^{ \{will,smith\} }]$};
			\node[main node] (2) [right = 3mm of 1] {$CASTING$};
			\node[main node] (3) [below = 3mm of 1] {$CASTING$};
			\path[draw,thick,->]
			(2) edge node {} (1)
			(3) edge node {} (1)
		} 
		& expand $1$, enqueue $2$ \\
		
		
		\hline
		$T_4$ &
		\tikz{
			\node[main node] (1) {$PERSON^V[name^{ \{will,smith\} }]$};
			\node[main node] (2) [right = 3mm of 1] {$CASTING$};
			\node[main node] (3) [right = 3mm of 2] {$MOVIE^S[self^{\{films\}}]$};
			\path[draw,thick,->]
			(2) edge node {} (1)
			(2) edge node {} (3)
		}
	& 
	return generated CN	\\
		\hline
	\end{tabular}
}

==> tables/tab_singleqjp_m2.tex <==
{\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|c|l|l|} 
		\hline
		\textbf{ I\# }  & \textbf{Queue }                                                                              & \textbf{Operations }                              \\ 
		\hline
		0                & $\langle PERSON^V[name^{ \{will\} }]\rangle$                                                            & initialize, enqueue~$0$                           \\ 
		\hline
		1                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ]\rangle$                                                  & expand $0$, enqueue $1$                           \\ 
		\hline
		2                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , PERSON^V[name^{ \{smith\} }] \rangle$ (pruned)         & expand $1$, enqueue $2$                           \\
		3                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , MOVIE^S[self^{\{films\}}]\rangle$                                          & expand~$1$, enqueue~$3$		\\
		4                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , PERSON^F[\ ]\rangle$ (pruned)                                & expand $1$, enqueue $4$                           \\
		5                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , CHAR^F[\ ]\rangle$                                           & expand~$1$, enqueue~$5$                           \\
		6                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , ROLE^F[\ ]\rangle$                                           & expand~$1$, enqueue~$6$                           \\ 
		\hline
		7                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , MOVIE^S[self^{\{films\}}] , CASTING^F[\ ]\rangle$                                & expand~$5$, enqueue $7$                           \\ 
		\hline
		8                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , CHAR^F[\ ] , CASTING^F[\ ]\rangle$                                 & expand~$4$, enqueue~$8$                           \\ 
		\hline
		9                & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , ROLE^F[\ ] , CASTING^F[\ ]\rangle$                                 & expand~$6$, enqueue~$9$                           \\ 
		\hline
		10               & $\langle PERSON^V[name^{ \{will\} }] , CASTING^F[\ ] , MOVIE^S[self^{\{films\}}] , CASTING^F[\ ], PERSON^V[name^{ \{smith\} }]\rangle$  & expand $7$, \textbf{return} $\mathbf{Q\!J_{2}}$   \\
		\hline
	\end{tabular}
}
